Representation Learning for High-Dimensional Data Collection under Local Differential Privacy

The collection of individuals' data has become commonplace in many industries. Local differential privacy (LDP) offers a rigorous approach to preserving privacy whereby the individual privatises their data locally, allowing only their perturbed datum to leave their possession. LDP thus provides a provable privacy guarantee to the individual against both adversaries and database administrators. Existing LDP mechanisms have successfully been applied to low-dimensional data, but in high dimensions the privacy-inducing noise largely destroys the utility of the data. In this work, our contributions are two-fold: first, by adapting state-of-the-art techniques from representation learning, we introduce a novel approach to learning LDP mechanisms. These mechanisms add noise to powerful representations on the low-dimensional manifold underlying the data, thereby overcoming the prohibitive noise requirements of LDP in high dimensions. Second, we introduce a novel denoising approach for downstream model learning. The training of performant machine learning models using collected LDP data is a common goal for data collectors, and downstream model performance forms a proxy for the LDP data utility. Our approach significantly outperforms current state-of-the-art LDP mechanisms.

==> tables/data_collection_feature_level.tex <==
\begin{table*}[t]
\caption{Data collection on feature level}
\label{tab:data_collection_feature_level}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{p{0.7cm}p{23.3mm}|p{15mm}p{15mm}p{15mm}p{15mm}p{15mm}p{15mm}|p{19mm}}
\toprule

& \makecell[l]{Mechanism}
& \makecell[c]{$\eps_\text{ldp}=10$}
& \makecell[c]{$\eps_\text{ldp}=8$}
& \makecell[c]{$\eps_\text{ldp}=6$}
& \makecell[c]{$\eps_\text{ldp}=4$}
& \makecell[c]{$\eps_\text{ldp}=2$}
& \makecell[c]{$\eps_\text{ldp}=1$}
& \makecell[c]{No Privacy}
\hspace{0.5cm}
\\
\midrule
&VLM (rep. level)
&\textbf{86.1±1.0}
&\textbf{82.1±1.6}
&\textbf{72.8±3.2}
&\textbf{61.3±2.8}
&\textbf{35.3±9.7}
&16.9±1.3
&94.9±0.2
\\ %\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering MNIST}}}
&VLM (feature level)
&70.2±3.8
&64.4±4.9
&50.5±3.4
&45.6±0.9
&25.7±6.9
&19.5±9.1
&90.4±0.7
\\ %\hline
&PrivUnit
&38.2±4.6
&15.1±4.2
&12.4±1.6
&9.2±2.6
&9.5±2.9
&11.3±4.5
&96.0±0.4
\\ %\hline
&Duchi
&13.9±4.5
&14.3±5.0
&13.3±3.8
&14.1±4.9
&14.0±5.6
&10.0±1.1
&96.0±0.4
\\ %\hline
&Laplace
&\;\;9.2±1.4
&\;\;9.8±2.8
&10.6±0.3
&10.0±0.6
&\;\;9.0±1.1
&10.0±0.8
&96.0±0.4
\\ \hline
&VLM (rep. level)
&\textbf{63.7±0.6}
&63.2±0.3
&\textbf{62.6±0.5}
&61.1±1.2
&\textbf{53.9±4.3}
&\textbf{55.1±4.5}
&65.0±0.3
\\ %\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \;Lending Club}}}
&VLM (feature level)
&63.4±0.2
&63.3±1.0
&63.4±0.4
&62.1±0.4
&56.3±2.0
&52.7±3.3
&65.0±0.2
\\ %\hline
&Duchi
&56.0±5.5
&53.0±4.2
&52.7±2.9
&50.1±1.4
&50.1±0.9
&49.3±2.5
&65.7±0.2
\\ %\hline
&Laplace
&50.1±0.6
&50.3±0.8
&49.6±1.1
&49.7±1.2
&49.9±0.7
&49.5±0.9
&65.7±0.2
\\ \bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
